Gaussian-Based and Outside-the-Box Runtime Monitoring Join Forces

Since neural networks can make wrong predictions even with high confidence, monitoring their behavior at runtime is important, especially in safety-critical domains like autonomous driving. In this paper, we combine ideas from previous monitoring approaches based on observing the activation values of hidden neurons. In particular, we combine the Gaussian-based approach, which observes whether the current value of each monitored neuron is similar to typical values observed during training, and the Outside-the-Box monitor, which creates clusters of the acceptable activation values, and, thus, considers the correlations of the neurons' values. Our experiments evaluate the achieved improvement.

==> figures/gtsrb-manipulated-images.tex <==

    \begin{tabular}{cccc}
       \includegraphics[width=0.20\linewidth]{images/gtsrb/manipulated/original} & 
    \includegraphics[width=0.20\linewidth]{images/gtsrb/manipulated/new_world_cifar10} & 
    \includegraphics[width=0.20\linewidth]{images/gtsrb/manipulated/new_world_dtd} & \includegraphics[width=0.20\linewidth]{images/gtsrb/manipulated/gaussian_noise} \\
     \parbox{0.20\linewidth}{\centering\texttt{ID \\ Original}} & 
     \parbox{0.20\linewidth}{\centering\texttt{New World \\ CIFAR10}} &  
     \parbox{0.20\linewidth}{\centering\texttt{New World \\ DTD}} &
     \parbox{0.20\linewidth}{\centering\texttt{Noise \\  Gaussian}}\\ [1em]
    
    \includegraphics[width=0.20\linewidth]{images/gtsrb/manipulated/salt_and_pepper} & 
    \includegraphics[width=0.20\linewidth]{images/gtsrb/manipulated/contrast} &
     \includegraphics[width=0.20\linewidth]{images/gtsrb/manipulated/gaussian_blur} & 
    \includegraphics[width=0.20\linewidth]{images/gtsrb/manipulated/invert}  \\
    \parbox{0.20\linewidth}{\centering\texttt{Noise \\ Salt \& Pepper}} & 
     \parbox{0.20\linewidth}{\centering\texttt{Perturbation \\ Contrast}} &  
     \parbox{0.20\linewidth}{\centering\texttt{Perturbation \\ Gaussian Blur }} &
     \parbox{0.20\linewidth}{\centering\texttt{Perturbation \\ Invert}}\\ [1em]

    
    \includegraphics[width=0.20\linewidth]{images/gtsrb/manipulated/rotate} &
     \includegraphics[width=0.20\linewidth]{images/gtsrb/manipulated/light} & 
    \includegraphics[width=0.20\linewidth]{images/gtsrb/manipulated/new_world_chinese} & \\
     \parbox{0.20\linewidth}{\centering\texttt{Peturbation \\ Rotate}} & 
     \parbox{0.20\linewidth}{\centering\texttt{Perturbation \\ Light}} &  
     \parbox{0.20\linewidth}{\centering\texttt{Unseen Object \\ CTS}} & \\[1em]
  
    \end{tabular}


==> format/macros.tex <==
% == SECTIONS
\setcounter{secnumdepth}{3} 
\captionsetup[sub]{font=footnotesize}
\Crefname{subsubsubappendix}{Appendix}{Appendices}%

% == ALGORITHMS
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}


% == SYMBOLS

\RequirePackage{marvosym}

\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\DeclarePairedDelimiter\abs{\lvert}{\rvert}

% == BASIC SETS

\newcommand{\Naturals}{\mathbb{N}}
\newcommand{\Reals}{\mathbb{R}}
\newcommand{\Distributions}{\mathcal{D}}
\newcommand{\Paths}{\mathsf{Paths}}


% == OPERATORS

\DeclareMathOperator*{\argmax}{arg\, max}
\DeclareMathOperator*{\argmin}{arg\, min}
\newcommand{\post}{\mathsf{post}}
\newcommand{\eqdef}{\vcentcolon=}
\newcommand{\defeq}{=\vcentcolon}

\newcommand{\qee}{\hfill$\triangle$} % quod erat exemplandum % TODO del

% == PROBABILITY
\renewcommand{\Pr}{\mathbb{P}}
\newcommand{\Expectation}{\mathbb{E}}

% == MC, MPD, Games
\newcommand{\MDP}{\mathcal{M}}
\newcommand{\initstate}{\bar{s}}
\newcommand{\states}{\mathsf{S}}
\newcommand{\actions}{\mathsf{A}}
\newcommand{\trans}{\delta}
\newcommand{\gStates}{\mathsf{G}}
\newcommand{\Reach}{\mathsf{Reach}}
\newcommand{\domain}{\mathbb{D}}

% = paths and strategies
\newcommand{\apath}{\rho}
\newcommand{\paths}{\mathsf{Paths}}
\newcommand{\policy}{\sigma}
\newcommand{\policies}{\Sigma}
\newcommand{\prob}{\mathbb{P}}
\newcommand{\opt}{\mathsf{opt}}

% == Proof ideas
\spnewtheorem*{proofidea}{Proof Idea}{\itshape}{\rmfamily}



\newcommand{\val}{\mathsf{V}}


\newcommand{\orcidID}[1]{{\href{https://orcid.org/#1}{\protect\raisebox{3.25pt}{\protect\includegraphics{orcid_color}}}}}

\newcommand{\inlineheadingbf}[1]{\smallskip\noindent{\bfseries #1.}}
\newcommand{\inlineheadingbfd}[1]{\smallskip\noindent{\bfseries #1}}
\newcommand{\inlineheadingit}[1]{\smallskip\noindent{\it #1.}}


\newcommand\tool[1]{{{\scshape #1}\xspace}}
\newcommand\definetool[2]{\newcommand{#1}{\tool{#2}\xspace}}
\definetool{\monitizer}{Monitizer}
\definetool{\verinet}{VeriNet}
\definetool{\marabou}{Marabou}


\newcommand\cifarten{CIFAR-10\xspace}
\newcommand\gtsrb{GTSRB\xspace}
\newcommand\mnist{MNIST\xspace}
\newcommand\cifartennet{CIFAR-10-NET\xspace}


\newcommand{\relu}{ReLU\xspace}

==> format/tikz-defs.tex <==
\usetikzlibrary{shapes,positioning,arrows,calc,automata,matrix,fit}
\tikzstyle{state}+=[minimum size = 6mm, inner sep=0,outer sep=1]
\tikzset{->,>=stealth'}

%% -------------------------------------- Declare the layers
\pgfdeclarelayer{nodelayer}
\pgfdeclarelayer{edgelayer}
\pgfsetlayers{edgelayer,nodelayer,main,connections,background}


